SLEUTH: Real-time Attack Scenario Reconstruction from COTS Audit Data

We present an approach and system for real-time reconstruction of attack scenarios on an enterprise host. To meet the scalability and real-time needs of the problem, we develop a platform-neutral, main-memory based, dependency graph abstraction of audit-log data. We then present efficient, tag-based techniques for attack detection and reconstruction, including source identification and impact analysis. We also develop methods to reveal the big picture of attacks by construction of compact, visual graphs of attack steps. Our system participated in a red team evaluation organized by DARPA and was able to successfully detect and reconstruct the details of the red team's attacks on hosts running Windows, FreeBSD and Linux.

==> analysis.tex <==
%

\section{Approach}
In this section, we present our approach. The main goal of our system is to detect attacks by using a system's audit logs, which contain system calls and other information related to events. In addition to the detection, we want to provide complete information on the activities of an attacker inside the system, including the attack's entry point, corrupted processes, and modified or exfiltrated files. We focus on APT style attacks, whose majority has the following characteristics. 

\noindent
\textit{No insider threat}
The attacks are executed by some external entity. Therefore, there is at least an entry point to the system (we name such entry points as sources).

\noindent
\textit{Sensitive resources}
The attacker is interested in sensitive resources (changing password files, process corruption, exfiltrating information). Therefore we expect that there exists some observable access via the audit logs to these resources (we name such resources as sinks).

\noindent
\textit{Untrusted code execution}
In some way, the attacker manages to execute some malicious code inside the system. This may happen as part of a drive by download attack, as part of a spear phishing attack, or in other ways. The malicious code also produces events observable in the audit logs.

The types of attacks that we focus on are composed of a sequence of steps/events influenced by the attacker. These events are visible in the audit logs, however, they are mixed with a large number millions of other events produced by other benign processes. 

\subsection{Challenges}
There are several challenges that need to be overcome, in order to detect attacks using COTS audit logs.

\noindent
\textit {Scale}. The audit logs produce a large number of events, often at a rate of thousands per second. In order to process such a large data volume, we need to have an efficient way of representing, storing, and querying the information produced by these logs. We describe our solution to this challenge in Section \ref{sec:mainmem}. 

\noindent
\textit{Attack Detection} To detect an attack and all the activities at run time,  we must be able to pinpoint the events of the attack as soon as they happen. However, given the large scale of data, and the complexity of the audit data, isolating these events is not straightforward. We address this challenge, by using tag- and information-flow policies which are checked at run time. These policies are used to generate alerts about suspicious events. Once an alert is generated, the causes and the provenance of th alert are used to determine if it is part of an attack. We present the details of our solution in Section \ref{subsec:approach}.


%
\subsection{Approach}\label{subsec:approach}
We model the problem as a graph problem. Given a provenance graph G=(V, E, Li, Lc, F, A), where:
\begin{enumerate}
\item V is the set of vertices, representing processes, files, and sockets, ...
\item E is the set of edges representing events
\item Li is the set of integrity labels (untrusted, trusted, invulnerable)
\item Lc is the set of confidentiality labels (public, confidential, secret)
\item F: (V, E) -> (Li U Lc) is a label propagation function that assigns to each vertex an integrity or confidentiality label based on the incoming edge. The function F operates on nodes and edges in a streaming manner. It assigns labels based on the type of event, and on the labels of the previous events. It does, that is, the tag propagation.
\item A is a boolean function that assigns to each edge a boolean value that represents the fact that an alert has been associated with that edge or not. That is, every edge in the graph has an 'alert' attribute, which can be true or false. The function A, is based on policies, which represent suspicious events, that may have been influenced by the attacker. These include things like untrusted file execution, permission changes, reading of untrusted files, and so on. The function A is also computed in a streaming manner as nodes and vertices arrive.
\end{enumerate}

The problem is that of finding the subgraph Ga=(Va,Ea), representing an attack. Intuitively, an attack is a sequence of steps (paths in the graph) that:
\begin{enumerate}
\item contains at least one (?) edge with the alert value equal to 'true' (these are the alerts raised by SBU). That is there is at least one untrusted execute, or an untrusted load, and so on.
\item
	\begin{enumerate}
	\item starts at untrusted sources (nodes in the graph with indegree=0, such that their Li = untrusted), proceeds along a path where each vertex has Li >= LOW, and ends at sensitive sinks, that is at nodes in the graph with Li >= LOW. That is there is a path, influenced by the attacker, which reaches high integrity vertices. 
	
	\item and/or starts at high confidentiality sources (nodes in the graph, such that Lc>confidential) and ends at low integrity sinks.  
	\end{enumerate}
\item If there are multiple versions of the same entity along a path, they are ordered by increasing version number along the path (equivalently, the nodes along the path are ordered by increasing timestamp).
\end{enumerate}

The first condition captures single 'suspicious' steps of the attack (e.g., a downloaded file being executed, permission changes). However, by itself these suspicious steps are not sufficient to catch an attack. This is why we need a more global view, provided by the second condition.

The second condition, captures suspicious global information flow paths that contain at least one event influenced by the attacker, including information exfiltration. 

The third condition is not strictly related to the attack, it is more about discriminating the paths and looking only at those paths that are possible from a timestamp point of view. 


\subsection{Methodology}
\textbf{Challenge:} Scale. We can follow a traditional graph approach of finding paths between nodes in a graph. However, this is not efficient, in a graph of billions of nodes and edges. 

\textit{Solution}: pruning heuristiscs.

\textbf{Challenge:} The graph represents a live system. Therefore, it is continuously growing, with edges and nodes arriving in a streaming manner. Since our goal is detection of an attack, we need to efficiently compute the suspicious paths at runtime. This is complicated by the following observation. 
Suppose we see an alarm at a certain point in time t1. We cannot tell at time t1 if this alarm is related to a step of an attack or if it is just related to an innocuous operation (e.g., downloading a normal pdf file and reading it). To be able to say that this is an attack, we need to observe information flow from a source to the edge related to the alarm, and then from that edge to a sensitive sink. Such sensitive sink, however is not available at time t1, because the graph is growing.

\textit{Solution}: To address this challenge, we compute a provenance context at run time for every node. That is, for every node in the graph, we have the history of the information flow up to that node. 
This provenance context at the sinks helps us pinpoint immediately if there is a path from a source to the sinks and if there have been alarms generated along that path.

\subsection{Graph Pruning}
What we do is graph pruning. Motivation for graph pruning approach: The events related to an attack are a small minority of the overall events that are present in the trace/graph. Therefore, if we remove the events that are clearly not suspicious (that is nodes and edges that have the 'alert' value equal to false), we reduce the size of the problem by many orders of magnitude.

We use several pruning heuristics: \textbf{alert-based} pruning, \textit{Semantic-Preserving Filters}, \textit{Removal of Irrelevant/Unreachable Nodes and Edges}, \textit{Removal of Irrelevant Sources and Sinks}, and \textit{Removal of Nodes with High Integrity Tags}.

\subsubsection{Alert-based Pruning} We use output of function A to prune away the nodes that are clearly not part of the attack (show reduction rate in evaluation), because there is no information flow from the untrusted sources.  This is what SBU does. The result is a subgraph that contains edges with 'alert' equal to true and related nodes (in the provenance context). This captures the first condition. That is, we prune away everything that is not related to the alerts. \cite{}

\input{simplifications}



==> del.tex <==
\vtodo{Removed compactness section}
%
%
%
%
%
%
%
%
%
%
%
%
%
%

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%


Vertices in the graph represent objects (e.g., files and network connections) or
subjects (e.g., processes). For instance, when a process $p$
performs a write operation on a file $f$, this is captured by a directed edge
from $p$ to $f$. This edge denotes that $f$ depends on $p$ --- for instance, if
$p$ is compromised, we should suspect the integrity of $f$ as well. The edge is
annotated with the operation name and a timestamp, so that this information
could be output during an analysis.


in the number of nodes in the graph, whereas naive versioning . The reason for 



Clearly, there is no way for $v$ to become compromised unless it depends on some
other entity (e.g., an external network connection or a local file) that is
deemed compromised. However, if the entire set of dependences of $v$ is
unchanged by $e$, then the compromised status of $v$ won't be changed by $e$,
and hence there is no reason to generate a new version of $v$. Thus, we optimize
our version generation by examining whether an event $e$ generates a new
dependence for $v$. In particular, if $e$ originates at a vertex that is already
an ancestor of $v$, we skip the generation of a new version.

%
%

%

\begin{obs}\label{verobs2}
  Consider an entity $v$ that has no outgoing edge, i.e., no other entity
  depends on $v$. There is no need to create a new version of $v$, even
  when a new edge $e$ into $v$ is added that changes $v$'s dependence. 
\end{obs}

In this case, we may discover in the future that $e$ caused $v$ to become
compromised. However, this update to $v$'s status won't cause the state of
any other existing vertex to become incorrect or invalid, since nothing else depends
on the state of $v$.

These two optimizations are powerful in practice, especially in the case of
objects. In particular, they avoid generating multiple versions of objects in
the most common cases:

As a result, our versioning approach provides very good performance on objects,
%
limiting the increase (due to versioning) in the number of objects to less than 10\%.

Subjects tend to have more versions than objects, because any single subject
tends to interact with many objects. Still, the optimizations are effective in
reducing the number of versions in many common cases. For instance, processes
tend to load a large number of libraries initially. Each load represents an
inflow into the subject, and would require a new version with the naive
algorithm. However, because the subject typically performs no writes (i.e., no
new outgoing edges from the subject) during this phase,
Observation~\ref{verobs2} enables us to skip version generation. In our
experiments, we generate between 1.1 and 1.5 versions of each subject, on average.
This represents at least a 20-fold improvement over the naive approach.

\noindent Our versioning approach provides the following benefits:
\begin{itemize}
\item {\em Simplify impact analysis.} If any vertex in the graph is determined
  to be malicious (or compromised), the set of all vertices impacted by this
  can be quickly computed using a simple depth-first search from this vertex.
  In the unversioned case, a simple search will flag many unaffected vertices,
  while with our versioned approach, only those vertices that truly depend
  on the compromised vertex would be flagged. Alternatively, in the unversioned
  case, accurate impact analysis may be performed by maintaining timestamps
  with edges, and only following outgoing edges whose timestamps are greater
  than that of the incoming edge. However, this complicates the algorithm,
  while increasing the storage for edges.
\item {\em Speed up graph algorithms.} The versioned graph is acyclic (see
  Observation~\ref{verobs3} below). Algorithms on acyclic graphs can be
  simpler, as well as more efficient than general graphs.  For instance,
  linear-time shortest path algorithms are available for DAGs, but not for
  general graphs.
\item {\em Space savings via reduction in edges.} If objects and subjects were
  unversioned, then, in order to perform accurate impact analysis, we would
  need to maintain all of the events in the graph, together with their
  timestamps. In contrast, our versioned
  implementation avoids redundant edges. While the details about all events
  (concerning nodes involved in a compromise) may need to be presented to
  the analyst in the end, this information can be kept in secondary storage,
  while the graph itself is maintained in main memory.  
\end{itemize}
\hrulefill

\begin{obs}\label{verobs3}
Versioned graphs are acyclic.  
\end{obs}
{\bf Proof}  is by contradiction. Suppose
    that a cycle is present in the versioned graph. Consider the graph just
    before the first cycle is formed. Let the cycle consist of vertices $v_1,
    v_2,\ldots, v_n$.  Let the edge $e$ from $v_n$ to $v_1$ be the last edge
    that is added. When $e$ is added, note that Observation~\ref{verobs2}
    is not applicable because $v_1$ already has an outgoing edge to $v_2$. Moreover, if Observation~\ref{verobs1} is applicable, then $v_n$ would already
    be an ancestor of $v_1$. This means that there already exists a path from
    $v_1$ to $v_n$, and then from $v_n$ to $v_1$, contradicting the assumption
    that $e$ is the first edge that forms a cycle. Thus, Observation~\ref{verobs1} is also not applicable. Since neither observation is applicable, our
    algorithm will create a new version $v_1'$ of $v_1$, and hence the addition
    of $e$ will not result in a cycle\ep

\note{I think we don't need to talk about the following at all, since we
have a pretty convincing discussion about versioning. Since versioning isn't 
something that DBs do, it is not longer necessary to justify our choice.
Some of the points can be moved to implementation/evaluation, while the
note about inefficiency of DBs can be mentioned in the discussion of
memory usage of our system.}

%
%

%

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

%

%
%
%
%
%
%
%
%
%
%
%

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%



The attack scenario reconstruction is initiated by the following two alarms
generated by the tag-based detection component of \projname:\medskip

\begin{scriptsize}
  \begin{tt}
\noindent
16-09-09 09:28:37.832: Alarm: UntrustedLoad: Object \verb+C:\Users\User1\Downloads\firefox\dropper+\linebreak\indent
Subject pid=560 \verb+C:\Program Files\Mozilla\firefox\firefox.exe+\\[0.7ex]
16-09-09 09:55:07.049: Alarm: UntrustedLoad: Object \verb+C:\dropper+\linebreak\indent
Subject pid=1580 \verb+C:\Program Files\Mozilla\firefox\firefox.exe+
\end{tt}
\end{scriptsize}

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

\noindent
Given the above alarms, using forward analysis from the point of
these alarms, \projname reconstructed the attack graph shown in Figure \ref{fdbov1}.


%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

\comment{
Figure~\ref{memuse} shows the sizes and memory used for the data sets we
consumed and successfully analyzed. In summary, we make the following
observations:
\begin{itemize}
\item We first translate CDM into our common semantic representation (CSR),
  a uniform representation that we use across different OSes. CSR is stored
  in compressed (gzipped) format. On average, CSR is about
  40 times smaller than the binary representation used in CDM.
\item On average, we use about one byte of memory per CDM record for
  data from FiveDirections, and about 4 bytes per CDM record for data from {\sc Linux}.
\end{itemize}

\begin{figure*}[ht!]
 \begin{footnotesize}
  \begin{center}
  \begin{tabular}{||c|r|r|r|r|r||}
    \hline
    Data set & CDM  & CSR  & CSR/CDM & Main & Memory/ \\
             & size &  Size & ratio & memory& CDM ratio \\
    \hline \hline
    W-1 &  49 MB & 0.8 MB& 1.6\% & 0.6 MB & 1.2\%\\ \hline \hline
    W-2 & 150 MB  & 3 MB&  2.0\% & 2.1 MB & 1.4\%\\ \hline
    W-3 & 130 MB & 2.5 MB& 1.9\% & 1.7 MB & 1.3\%\\ \hline
    \multicolumn{3}{||c}{\bf Windows Mean}  & {\bf 1.9\%} & \multicolumn{2}{|r||}{\bf 1.3\%}\\ \hline\hline
    \ts L-1 & 13 GB & 0.4GB& 3.1\%& 0.7 GB & 5.4\%\\ \hline \hline
   \ts  L-2 & 175 GB & 4.7 GB& 2.7\% & 11.3 GB & 6.4\%\\ \hline
    \ts L-3 & 111 GB & 3.9 GB& 3.5\% & 5.8 GB & 5.2\%\\ \hline
    \multicolumn{3}{||c}{{\bf {\sc Linux} Mean}}    & {\bf 3.1\%} &  \multicolumn{2}{r||}{\bf 5.7\%}\\ \hline
  \end{tabular}
\end{center}
  \end{footnotesize}

  \caption{Size of main memory provenance graph and common semantic
    representation (CSR). ``CDM size" refers to the size of CDM binary format,
    as stored in Kafka queues. CSR is stored in gzipped text format.} \label{memuse}
\end{figure*}
}
%
%
\subsubsection{Runtime}
%
\paragraph{Graph Construction}

\comment {In this section, we focus on how much automation is brought to the forensic
analysis by our techniques. In particular, attack detection is automated, and
it identifies the most suspicious events. Starting from these events, \projname
performs an automated forward analysis. During this analysis, configurable
policies are used to filter out uninteresting events performed by suspect
processes (e.g., loads of benign libraries), while retaining significant events.
This results in a very small fraction of the CDM events being flagged for
further analysis.

In some cases, the filtered event set is small enough to be directly fed into a
graph visualization program such as {\small \tt graphviz}. In other cases, the number
of events is too large, and is subject to further manual analysis.
Figure~\ref{selectivity} shows how selective these automated processes are. Less
than one-thousandth of the CDM events are flagged for further analysis.
}
%
%
  %
  %
    %
    %
      %
    %
     %
    %
   %
     %
     %
     %
  %
  %
  %
  %
%




  \begin{figure*}[ht!]
  \begin{footnotesize}
  \begin{center}
  \begin{tabular}{||c|c|c|c|c|c|c|c|c||}
  \hline
  \multirow{2}{*}{Dataset} &\multirow{2}{*}{Events} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}UntrustedExec\\ Alarm\end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}WriteByLowInteg\\ Alarm\end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}PermChngForExec\\ Alarm\end{tabular}} & \multicolumn{2}{c||}{\begin{tabular}[c]{@{}c@{}}ConfDataLeak\\ Alarm\end{tabular}} \\ \cline{2-9} 
       & \multicolumn{1}{c|}{Naive}   & \multicolumn{1}{c|}{\projname} & \multicolumn{1}{l|}{Naive}  & \multicolumn{1}{c|}{\projname} & \multicolumn{1}{c|}{Naive} & \multicolumn{1}{c|}{\projname} & \multicolumn{1}{c|}{Naive} & \multicolumn{1}{c||}{\projname}  \\ \hline
    \ts  W-1   & 21    & 3  & 1 K     & 3     & 0    & 0   & 6.1 K    & 11  \\ \hline 
    \ts  W-2   & 44    & 2  & 1.4 K   & 108   & 0    & 0   & 25.3 K   & 18  \\ \hline \hline
     \ts L-1   & 60    & 2  & 53      & 5     & 1    & 1   & 19       & 6     \\ \hline
    \ts L-2    & 1.5 K & 5  & 19.5 K  & 1     & 280  & 8   & 122 K    & 159   \\ \hline
    \ts L-3    & 695   & 5  & 26.1 K  & 2     & 270  & 0   & 62.1 K   & 5.3 K \\ \hline
  \end{tabular}
  \caption{Comparison of generated alarms} \label{alarm}
  \end{center}
  \end{footnotesize}
  \end{figure*}

%


that there is an

important for an enterprise security operations analyst
to detect, {\em in real time}, whether an attack occurred, and if so, 
pr
how the
attacker obtained access to the system and what the impact is. While existing
tools can be helpful in detection, they do not 

Yet, there is
very little by way of support in commodity operating systems that assist the
analyst in detecting the chain of events leading to an attack.

The main issue is one of scale: at any given point, there is an enormous volume
(i.e., millions or billions of records) of data collected in the system through
the system's audit logs --- but only a tiny fraction (say a few hundred records)
of this data is involved in the actual attack. Thus the security analyst is
looking for a real-time solution to this ``needle-in-haystack'' problem --- a
system that can prioritize events, stitch them together in real time, as events
are unfolding; and present scenarios that an analyst can understand and act on.

In an enterprise, the security analyst does have a number of real-time detection
tools at his/her disposal such as Intrusion Detection Systems, Security
Information and Event Management (SIEM) tools, identity and access management
tools, application security tools, and application firewalls. While these tools
are generally useful in generating real-time alerts in the event of an attack,
they tend to generate a multitude of them over a sufficiently long period,
without giving the analyst a compact summary of the causal chains that lead to
the attack. The analyst is now faced with the tedious challenge of analyzing
these alerts manually. In recent high-profile incidents, similar reasons have
led analysts to ignore these alerts~

%



 that addresses
these challenges. At a high level, our approach develops both
representations and methods for reasoning about COTS event data in real-time to
produce compact, visual scenarios of attacks.

In our threat model, we assume that such an attack originates externally.
This could mean an 

%

Its components incorporate several key ideas to tackle the four
challenges mentioned earlier. 

%

Our graph model . In order to make the
analysis procedures efficient, we store this graph compactly in main memory in
order for our algorithms to process them efficiently. This allows \projname to
achieve a significant speedup in the data consumption and graph analysis, with
respect to off the shelf graph databases used in big data analysis, which have
to resort to disk storage with very large datasets (e.g., \cite{neo4j}).

%

\projname is different from other alert correlation
efforts~\cite{debar2001,ning2003,qin2003,noel2004,wang2008,pei2016hercule} that
rely mainly on machine learning or other statistical techniques. Instead, we
have based our approach on tags and provenance tracking. Although our current
implementation is based on audit data, it can leverage additional precision
offered by fine-grained tracking approaches
\cite{newsome05,usenix06,yin2007panorama,egele2007dynamic,kim2010intrusion,
lee2013high,angelos} to provide enhanced accuracy. %
                                                   %
%
%
%
%
%
%
%
%
%
%
%

%

\newcommand{\ra}{\rightarrow}
\begin{table}[ht!]
  \begin{center}
    \begin{adjustbox}{width=0.9\columnwidth}
       \begin{tabular}{||c|c|c|c||}
       \hline
       Event   & Direction & Alarm & Tag value \\
       &     & trigger & trigger \\
       \hline
       {\tt define} & & I ($init$) & \\
       \hline
       {\tt read}   & O$\ra$S & R ($read$)         & $propRd$\\
       \hline
       {\tt load}, {\tt execve}   & O$\ra$S & E ($exec$) & $propEx$\\
       \hline
%
%
       {\tt write}  & S$\ra$O & W ($write$)         & $propWr$\\
       \hline
       {\tt rm}, {\tt rename}     & S$\ra$O & W       &      \\
       \hline
       {\tt chmod}, {\tt chown}  & S$\ra$O & W, M ($modify$)  &      \\
%
%
       \hline
       {\tt setuid} & S$\ra$S &            & $propSu$\\
       \hline
       \end{tabular}
       \end{adjustbox}
    \end{center}
  \caption{Edges with policy trigger points. In the direction column, S
    indicates subject, and O indicates object. The next two columns indicate
    trigger points for alarm and tag setting policies.}
  \label{fig:event-type}
\end{table}

%


fully implemented, so the data we used in
our analysis was very much at the level of OS audit logs. Specifically,

 or were unavailable to us because
of interface li


 that involves research
teams from academia and industry There were several teams dedicated to
producing audit data, while other teams, such as ours, were concerned with
attack detection and forensics.


  
\rtodo{Merged previous table about the dataset with table about distribution
  (Previous table is commented in the latex source).}

%
%
%
%
%
%
To produce audit data, the Linux team relied on the 

%

We evaluated \projname with audit data from three teams, covering Linux, FreeBSD
and Windows hosts. The red team carried out 8 attack campaigns across these
three platforms. The audit data 

%

As
shown in Table \ref{tab:dist}, there are 2 campaigns on Windows hosts (W-1 and
W-2), 3 campaigns on Linux hosts (L-1, L-2, and L-3), and 3 campaigns on FreeBSD
hosts (F-1, F-2, and F-3). {\color{red} The data were being produced by the
  other teams and sent to our team in real time. \projname was consuming,
  storing in memory and analyzing these data to extract the attacks in real time
  as well.}


%


%
%
%
%
%
The remaining scenarios are deferred to 

%




 that we had identified as part of the attack, but they weren

correspond to false positives. But they 

 we only included those key entities were
actually mentioned in the audit data. 


We examined
these misses carefully. In almost every case 


One of the misses
concerned a sensitive file that we failed to catalog, and the other miss
concerned an important device file. 

as a prototype system,
\projname had not been put through a careful phase of identifying
 sensitive data files, or 
all the important device files. 


{\color{red} In campaign F-1, we missed one portion of the attack
because some files were not labeled sensitive initially. After labeling 
these files, and consuming the data again, the attack was detected. In the same campaign, 
we identified a recompilation of the {\tt nginx} server as an attack. However, we verified from
the ground truth that those activities were part of post-engagement restoration
of the nginx server, and the auditing was (mistakenly) turned on during this
process.}


of main
memory to store the data of one day, and less than 40 seconds to analyze them
and construct the attack scenario. To store the data for a period of, say, 6
months, a simple extrapolation suggests that \projname would require only 18GB
of main memory, well within the limits of today's commodity hardware. As a
result, memory use can be as small a


==> intro.tex <==
%

\section{Introduction} \label{intro}
%
We are witnessing an ongoing spate of targeted cyber-attack activities conducted by skilled adversaries. 
%
Yet, there is very little by way of support in commodity operating systems towards identification and attribution of these attacks, leaving these jobs to a handful of specialized firms that employ skilled security professionals for these efforts. Through these (largely human-assisted) efforts, we have seen a number of intelligence reports~\cite{apt-reports} that have shed light on these attack scenarios that characterize the intent and methods used by these adversaries. However,  commodity operating systems are yet to provide first-class automatic support not only for attack detection (i.e., reporting whether an attack occurred), but also for attack scenario reconstruction (i.e., how the attacker gained access and what the impact is). 

%


%
%

BackTracker was one of the first approaches to study the problem of reporting 

There has been considerable progress on the inclusion of software protection  measures in mainstream OSes, most notably ASLR and DEP. However, the ongoing increase in the number and variety of targeted attacks suggests that adaptive adversaries that can evade these protection and prevention mechanisms through mechanisms like spearphishing. This has pushed the burden on enterprises to rely more on second-line defenses, e.g., the use of perimeter-based controls such as firewalls, IPS/IDS, SIEM tools, identity and access management tools, application security tools, and application firewalls. While these tools are generally useful, they generate a multitude of event alert streams as well as logs and audit records, sometimes in their own custom formats. These logs  contain potentially actionable intelligence, but there are no techniques available that work with diverse OSes to consolidate and correlate individual reports of suspicious behavior into a coherent scenario or campaign and present them in a semantically-meaningful manner to the security analyst.

We address this problem in this paper. At a high level, our approach develops both representations and methods for reasoning about COTS audit data in order to produce meaningful security reports.  Our approach is based on the application of information-flow tracking techniques to audit logs to construct and analyze platform-neutral dependence graphs.  The high-level analysis goals are to (a) detect attacks, (b) identify the sources of attacks, (c) perform impact analysis to identify the complete effects of attacks, and (d) present summaries of attacks in a meaningful visual abstraction.  Our analyses for (b)-(d) can be applied to attacks detected by our own approach, other tools, or manual efforts.

Our dependence graph is platform-neutral and has allowed our implementation to process audit records from three commodity OSes.  On this graph, we define efficient methods for tracking down the actions of adversaries through coarse-grained information flow tracking. Our tracking methods use tags (also called labels) to indicate trustworthiness and confidentiality. These tags are initialized and propagated using a powerful policy framework that assists in curtailing, in a principled and application-independent way, common situations that lead to extraneous or irrelevant subjects or objects in the final report.  Using these policies, our system produces alarms that indicate policy violations. 

%

%
%
%

%
%

%


%

  
\paragraph{Contributions} The main contributions of this paper are:
\begin{itemize}
\item provenance-based attack detection technique with very low false
positives and false negatives
\item accurate provenance-based attack reconstruction technique, including
source identification and impact analysis, with effective filtering to
remove extraneous events
\item both techniques require only COTS audit data and are
platform-neutral, real-time, and high-performance
\item flexible framework that supports customized policies for provenance
tracking and attack detection
\end{itemize}


Our approach is implemented in a system called \projname (attack Scenario LinkagE Using provenance Tracking of Host audit data). \projname  was evaluated on a government-agency led red team evaluation that conducted  attacks on Windows, FreeBSD and Linux hosts over a two week period. Our system was able to: 1) process in a matter of seconds audit logs containing millions of events generated by over 100 programs over several days; 2) successfully detect and reconstruct the details of these attacks, including their entry points, activities in the system, and exfiltration points; 3) filter away extraneous events achieving very high reductions rates in the data (up to more than 100 thousand times), thus providing a  clear semantic representation of these attacks containing almost no noise from other activities in the system; and 4) achieve a  low false positive and false negative rate.  While we have evaluated the system primarily in a forensic setting, the performance of \projname makes it suitable for attack detection in real-time. 


This paper is organized as follows.  Section~\ref{sec:overview} provides a high-level overview of the approach. Sections~\ref{sec:detection} through~\ref{sec:forensics} discuss the components of the system in detail. In particular, Sec~\ref{sec:detection} discusses the design of tags and their use in detection. In Section~\ref{sec:graph}, we discuss the graph model and policies.  Our backward and forward analyses for attack scenario reconstruction are described in Section~\ref{sec:forensics}. Section~\ref{sec:eval} presents an evaluation of the approach that includes discussions on effectiveness, performance and gap analysis and discusses the attack scenarios uncovered in the red-team evaluation.
Section~\ref{sec:relw} discusses background and related work. In Section~\ref{conclu}, we conclude. 

%
\comment{
The goal of this proposal is to investigate technologies that can
radically harden enterprise security by automating the tasks of
detecting, remediating and subsequently preventing sophisticated cyber
exploits. To this end, we explore if and how the ubiquitous knowledge
of provenance, in terms of causal linkages of activities in an
enterprise can be used along with big data techniques to mount a
better defense against the insidious attacks that thwart current
defenses and afflict enterprises today.

Enterprises today, largely use perimeter-based controls for their
defense such as firewalls, IPS/IDS, endpoint and server security
systems, SIEM tools, identity and access management tools, application
security tools, application firewalls and database firewalls.

So, while these tools generate a multitude of event alarm
streams as well as logs and audit records that contain potentially
actionable intelligence, they are typically not fully mined nor
available in real-time. The inability to consolidate and correlate
these events and data automatically at line speeds and present them to
the security analyst in a semantically-meaningful manner robs security
analysts and administrators of a valuable tool to defend enterprise
networks.
}

%
\comment{
Research on intrusion detection systems (IDS) was based on the following
assumption: there will always be attacks that get through the protection
mechanisms; and that the best one could hope for is to detect these {\em
  intrusions.} Being the last line of defense, IDS research accepted the need
for significant human involvement in reviewing, understanding and responding to
IDS reports. This factor, combined with a low tolerance for missed attacks,
promoted designs that generated a large volume alarms. Moreover, the alarms were
difficult interpret because they lacked sufficient context or specificity.
Consequently, these systems weren't particularly successful in terms of
practical adoption.

In the early 2000s, many security researchers began to question their
preoccupation with intrusion detection. Perhaps it was premature to focus on
detection at a time when so little had been done to build systems that resist
intrusions in the first place. Software vendors started paying much more
attention to security, reviewing and rewriting OS code, integrating
vulnerability mitigation mechanisms such as ASLR and DEP, and streamlining the
process for development and distribution of software patches. Researchers began
to focus on principles and techniques for developing secure software, as well as
vulnerability-specific defenses that could be (more or less) fully automated.
Simultaneously, a new-found emphasis on offensive research emerged, centered on
reverse engineering and the development of attacks, not only on benign
systems but also on malicious software and networks.

While traditional IDS research has languished over the past 10+ years, the
threat landscape has changed dramatically. The incentives and resources
available for carrying out attacks have grown exponentially. Attackers routinely
overcome deployed defenses, thus validating the assumption behind IDS. The
pendulum has swung back, but unfortunately, IDS techniques, which were already
difficult to use a decade ago, aren't up to the challenge posed by today's
systems that are far more complex. No one should be surprised today by the
frequency of high-profile intrusions, or the fact that many of them go
undetected for months or years.
}







==> overview.tex <==
%

\section{Approach and Challenges}
\label{sec:overview}
 \vspace*{-1ex}

%
In our problem setting, the goals of an attacker are to carry out an attack
campaign on an enterprise host system in order to exfiltrate confidential
information, corrupt assets or to simply maintain presence for a longer
duration. In our threat model, we assume that that such an attack originates
externally. This could mean an adversary could start the attack by hijacking a
web browser through externally supplied malicious input, or by supplying a
zero-day exploit to a network server run by the host. We assume that the
adversary has not implanted persistent malware on the host in advance of the
start of the detection mechanism (as otherwise his goal then would have been
already accomplished). We also assume that OS kernel and the audit system 
are trustworthy.

\begin{figure}[ht!]
  \vspace*{-1em}
  \begin{center}
    \hspace*{-2.5em}
    \includegraphics[width=1.15\columnwidth]{figures/nbuildinj-weighted}
  \end{center}
  \vspace*{-1em}
    \caption{Graph visualization of attack in running example.}
    \label{fig:buildinject}
\end{figure} 


\paragraph{Running Example.} 
%
We first discuss an example that illustrates the goals of our approach. In this
example, the goal of the attacker is to insert a backdoor in software developed
by members of a software development firm. As a first step, the attacker
exploits a Firefox process that visits a website hosted at \mytt{129.55.33.44}.
The browser process downloads an object file called \mytt{crt1.o} in the
filesystem under the home directory of the user Bob. The exploit also modifies
Bob's \mytt{.bashrc} file to create an alias for the \mytt{sudo} command. When
Bob subsequently runs \mytt{sudo apt-get}, elevated privilege is used by the
aliased \mytt{sudo} command to overwrite \mytt{/lib/crt1.o} with the downloaded
(malicious) version of \mytt{crt1.o}. Subsequently, Alice compiles and links a C
program. The resulting binary is malicious, because the loader automatically
inserts \mytt{/lib/crt1.o} into every executable.

%
 
Figure~\ref{fig:buildinject} illustrates the type of graph constructed by our
approach, taking as input the data from the auditing system running in this
host. Ovals, diamonds and rectangles represent processes, sockets and files,
respectively. Edges indicate dependencies between them. Our algorithm would omit
the dashed edges and their source nodes; we include them to illustrate the
overall scenario. The graph captures all of the attack steps and includes almost
no extraneous vertices and edges. Edges that propagate the attacker's actions
are colored in solid (red). 
%
%
%
Note that reconstructing the entire attack scenario in a visual manner is
critical for understanding the attack.

\note{Explain what the 1s and 0s mean in the figure}

\begin{figure*}[t]
\centering
    \includegraphics[width=\textwidth]{figures/architecture-new}
%
    \caption{System Architecture \label{fig:architecture}
    }
\end{figure*} 


\paragraph{Approach Goals.}
%
The goal of our approach is to analyze and detect threats to a host by examining
COTS audit logs, and flag malicious activities. The analysis should provide
actionable information --- in particular, we want the analysis to achieve the
following objectives in a system that operates in real time:
%
\begin{enumerate}[label=(\alph*)]
%
\item {\em Source identification:} Identify the external source (e.g. remote IP
  address and port) that served as the attack source or entry point, 
%
\item {\em Impact analysis:} compute the impact of the attacker's activities in
  the system, e.g., identify files modified and/or information exfiltrated.
%
\item {\em Attack visualization:} Generate and provide a graphical view of the
  attacker's activities in a form that is easily understood by a security
  admin/analyst,
%
\end{enumerate}
%
%
%
%
%
%
%
%
\paragraph{Technical Approach.} 
%
The main components of our approach are shown in Figure~\ref{fig:architecture}.
In our approach, we capture the information in the audit logs in the form of a
dependence graph. The vertices in the graph are objects (e.g., files and network
endpoints) and subjects (processes), while edges represent dependence. To
support real-time detection, we store this graph in main memory. We have devised
a compact representation for this dependence graph, enabling us to store
\note{provide example of sizes involved}.

A core technique in our approach is the use of tags with objects and subjects.
Tags capture our judgment about the trustworthiness and sensitivity of objects
and subjects. 




We also assign
confidentiality tags (c-tags) and integrity
%
tags (i-tags) to subjects and objects, and propagate these tags concurrently
when the graph is being constructed. These tags are propagated by rules that
correspond to the underlying coarse-semantics of the audit log
records.~\footnote{There is nothing inherent in our approach that is related to
  coarse-grained tracking, we can use finer granularity tracking if it is
  available.}




Our system also makes use of  detectors that identify specific nodes in the graph as malicious/compromised. Our implementation makes use of one such detector that is based on reasoning with policies expressed on event types and the tags of the associated subjects/objects.  Specifically,  tags allow us to associate a level of trustworthiness of subjects/objects, and enables us to
reason about whether a certain action is reasonable or not. 

Starting from these alerts, the analysis must proceed towards achieving the above-mentioned three objectives. In particular, starting from an alert location we perform bi-directional traversals of the graph. The backward traversal proceeds from an alert location and goes backward in time towards identifying the source or the entry point of the attack that generated the alert, meeting goal (a) above. A naive backward traversal will follow the chain of dependencies in the dependence graph. However, this will lead to a large subgraph that includes the entry point and the alert, one that includes many redundant edges. For instance, in our running example above,   the naive backward traversal will generate a subgraph that  includes  reads of many system files (e.g. \mytt{/etc/passwd} by sshd), when they are executed, but nevertheless, do not contribute to the main attack steps.  In general, this is the problem of dependence explosion or confusion, where activities that are not central to the attack get captured in the attack graph. We introduce several techniques that mitigate this problem to produce compact, workable graphs.

We tackle this first by defining a search model that prioritizes finding paths that represent actions of potential attack versus more benign operations from the system. In our backward search, if a node has incoming edges from multiple nodes with different trustworthiness tags, we follow only the edges leading to the predecessors with the lowest  value. This is done by assigning weights to edges in the dependence graph:  a zero weight to those backward edges that represent trustworthiness levels lower than the current node, and searching for  shortest paths (i.e. ones with least cost) in this weighted graph. The strategy identifies paths controlled by the attacker to reach the alert location while avoiding many  dependencies on typical  benign activities in the system. More on our search is discussed in Section~\ref{sec:forensics}.


Such backward searches on graphs are most efficient when there are no cycles in the graph. We achieve this through an acyclic graph representation. (This is in contrast to earlier works~\cite{king2003backtracking,king2005enriching} in this area that produce  cycled graphs.) In our representation, we achieve acyclic graphs by using an intelligent versioning system for subjects and objects, which we discuss in Section~\ref{sec:mainmem}. Such an  acyclic representation avoids the problem of dependence confusion, which is important to avoid with offline detectors. For example, a compromised node may be flagged a long time after the
 node and its descendants are constructed in the graph. More on our acyclic representation is discussed in Sec~\ref{subsec:versions}. A second important benefit of the DAG nature of our dependence graph is that   many graph algorithms (including shortest path) are faster on DAGs in comparison to those in cyclic graphs. This allows our search to be very efficient and makes our approach suitable for online analysis.  In particular, we can start the shortest path search from a compromised node, following edges backward, but pruning off  edges that don't lead to a descendant of an untrusted network  connection node.


 To further tackle dependence confusion, we split the trustworthiness tags assigned to subjects into two: one for its code trustworthiness (code t-tags) and the other for its data trustworthiness (data t-tags). Code trustworthiness involves tracking whether a subject has loaded untrustworthy executable code, whereas data trustworthiness  refers to whether a subject has read untrusted data. Code trustworthiness allows us to compactly identify actions of untrusted process executions. A naive forward dependence from detection point versus tracing those activities performed  	by subjects with untrusted code trustworthiness often can result in a three order of magnitude increase.  Trustworthiness tags are discussed in more detail in Section~\ref{subsec:tags}.

Finally, our presentation layer includes a number of simplifications that result in compact graphs. These rules do not change the basic characterization of the attack scenario that is uncovered, but they improve the visual aspect of it. Examples of such simplifications include, removal of unreachable and irrelvant nodes and edges,  and summarizing repeated events. These are discussed in more detail in Sec~\ref{sec:simplifications}. 

Despite the presence of these measures, there will still be benign dependencies in any system that cannot be ruled out through all the above methods. For instance, consider the file \mytt{.bash\_history} that is written by bash on every execution of the command. Inclusion of this file in the dependency chain could include a large number of dependencies that are irrelevant to the attack.    In this case, our approach includes a powerful policy architecture that provides a way for   customized policies to limit dependence   through objects like \mytt{.bash\_history}. The idea is to define a custom tag propagation policy for bash that leaves \mytt{.bash\_history} from being marked low trustworthiness. It is worth pointing out that  our approach  implementation handles the main subtleties in this example as code/data trustworthiness tags alone does not help because bash is an interpreter, so we need to treat file reads as loads, but doing so will downgrade bash to a low trustworthiness process. In general, custom policies identify interpreters and apply specialized labeling rules.  Our policy architecture is described in detail in ~\ref{sec:policy}.

%
%

%
%
%
%
%
%


%



%
%
%
%
%
%
%

%
%

%
Efficient analysis is an important concern in any online analysis system.  We therefore seek an efficient graph representation of audit log data that captures dependence information accurately. Such a representation is critical for developing efficient analysis techniques. Specifically, we wish to provide analysts and IDSs with the ability to mark suspicious nodes
%
in the graph at any time, and analyze their source and impact quickly. Since the graph can be extremely large (hundreds of millions if not billions of nodes), forensic analysis needs to operate in sublinear time --- specifically, the analysis needs to quickly identify a small subgraph that is relevant for the attack, and employ efficient algorithms on this subgraph. Ideally, the total time spent will be linear in the size of this subgraph.

We address this challenge  by developing a representation of the dependence graph in main memory. We develop a compact representation and use a variety of compression techniques to achieve compact storage. Since the algorithms operate on main memory, they achieve very good performance. For instance, the largest dataset  considered in our evaluation has over 2B edges and we are able to perform analysis on this dataset in a matter of seconds. We discuss our main memory representation in Section~\ref{sec:mainmem}.






%
%

%
%
%


%
%
%

%
%
%
%
%

%
%
%
%
%
%
%

%
%
%
%
%
%
%
%
%
%



%
%
%
%
%
%
%

%
%
%

%


%
%
%

%
%
%
%
%

%
%
%
%
%


==> tags.tex <==
\section{Integrity and Confidentiality Tags}
%
Many of our detection and forensic analysis algorithms rely on assignment and
propagation of tags. There are two types of tags: integrity tags and
confidentiality tags. Integrity tag values currently supported are:

COMPROMISED, UNTRUSTED, UNTRUSTED\_AUTHENTIC, BENIGN, BENIGN\_AUTHENTIC,
INVULNERABLE, WHITELIST

When the system boots up, sshd and any other processes that need to interact
with untrusted sources without getting downgraded themselves will be classified
as INVULNERABLE. Most other processes will run as BENIGN\_AUTHENTIC. This means
that most files on the system will also be labeled this way. (BENIGN\_AUTHENTIC
means that a source is benign, and strongly authenticated.)

The level BENIGN was created because the ta4 and ta5 scenarios involve attackers
logging in through legitimate ways (eg ssh) after stealing passwords (which we
don't know). So, a work-around was created to prevent these logins from being
classified as BENIGN\_AUTHENTIC. Specifically, a set of remote login programs
need to be specified. Whenever these programs perform a setuid, which usually
signifies the completion of a login, the integrity level is set to BENIGN.

Intranet sources would typically be tagged BENIGN, while most internet sources
will be tagged UNTRUSTED. Other integrity tag values are currently unused.

We also have the following confidentiality levels:

SECRET, SENSITIVE, PRIVATE, PUBLIC

SECRET is used for passwords, ssh keys, and the like. SENSITIVE is the next
level, but this level too is not used widely. Typically, selected files in
/var/log, /etc and /proc will be tagged sensitive. Most binaries and libraries
will be classified as PUBLIC, signifying the fact that they can be easily
obtained from public sources.

Tag propagation semantics is standard: if information with a tag t flows into an
entity E with a tag t', then E's tag will be downgraded to t if t < t'. For
integrity tags, the lowest integrity level is COMPROMISED, while the highest tag
that is normally used is BENIGN\_AUTHENTIC. For confidentiality tags, the lowest
level is SECRET and the highest level is PUBLIC.

Each subject has three tags: a code integrity tag, a data integrity tag, and a
data confidentiality tag. An object has two tags: a data integrity tag, and a
data confidentiality tag.

